Receptive-field-constrained stimulus optimization for human early and intermediate visual cortex

An ongoing challenge in sensory neuroscience is to characterize the feature dimensions encoded by cortical populations. Recent approaches probe feature selectivity in a data-driven way, by synthesizing a most-exciting-input (MEI) for a target neural population. While this approach has been successfully applied to human higher visual cortex using fMRI data, generating MEIs for early- and mid-level retinotopic visual areas requires additional modeling constraints due to small receptive field sizes. To address this challenge, we introduce two novel MEI generation frameworks, Receptive Field Diffusion for Visual Exploration (RF-DiVE) and Receptive Field Gradient Optimization (RF-GO). Both methods use a population receptive field (pRF)-constrained voxelwise encoding model; RF-DiVE combines this with a pretrained latent diffusion model, while RF-GO uses regularized gradient ascent. When applied to single voxels in retinotopically defined areas V1-hV4, using data from the Natural Scenes Dataset, we obtain MEIs that exhibit consistent structure within the pRF, suggesting selectivity for local features like contour, color, and texture. We systematically compare MEIs generated by RF-DiVE and RF-GO using two encoding backbones, performing in-silico validation of predicted responses to MEIs using independent encoding models. Across all methods and all visual areas, MEIs elicit higher model-predicted responses than the most activating natural images. We further find that the choice of generation framework and encoding backbone differentially affects MEI properties, including their visual appearance, structural interpretability, and cross-model generalizability. These results offer a new approach for performing data-driven characterization of spatial and feature selectivity across human visual cortex.

==> sections/07_extras.tex <==
\section*{AI Use Statement}
AI tools were used to assist with text polishing, code editing, computational job execution, and figure formatting. All code, scientific analyses, results, and interpretations were reviewed and verified by the authors.

\section*{Ethics Statement}

In this work we used human participant data encompassing fMRI measurements from the Natural Scenes Dataset \citep{allen2022massive}. The human participants procedures were approved by an appropriate Institutional Review Board as described in the original data paper. The data was shared in an anonymized format. We also collected new human behavioral data from online participants using Prolific. Participants provided informed consent, and the study procedures were approved by the Institutional Review Board at the authors' institution. Our research addresses basic science questions, and we do not anticipate any direct negative societal harm associated with these results.

\section*{Reproducibility Statement}

All details needed to reproduce our data processing steps and modeling procedures are provided in the main text (see \textit{Methods} and \textit{Experiments}) and in the Appendix. We plan to publicly release the code in the future.
% Note once we put the code online we can modify this to have a link to code. For now just have this.

